Functionalized few-layer silicene nanosheets: density functional theory on stability, structural, and electronic properties

Using density functional theory calculations, we investigated the properties of few-layer silicene nanosheets, namely bilayers and trilayers, functionalized with group-III or group-V atoms of the periodic table. We considered the Si$_2$X$_2$ bilayers and the Si$_2$X$_4$ trilayers, X = B, N, Al, P. We computed the structural, energetic, dynamic, elastic, and electronic properties of those systems in several stacking configurations, labeled as AA$'$, AB, AA$'$A$''$, and ABC. The results revealed that AA$'$-Si$_2$N$_2$, AB-Si$_2$N$_2$, AA$'$-Si$_2$P$_2$, AB-Si$_2$P$_2$, ABC-Si$_4$B$_2$, ABC-Si$_4$Al$_2$, AA$'$A$''$-Si$_4$P$_2$, and ABC-Si$_4$P$_2$ nanosheets are all dynamically stable, according to their respective phonon dispersion spectra. Additionally, by comparing the standard enthalpies of formation of doped few-layer silicene systems with the ones of the pristine silicene monolayer, bilayer, and trilayer nanosheets, we found that those structures could be experimentally accessed. Exploring the electronic properties of those stable systems, we discovered that the silicene bilayers and trilayers functionalized with N or P atoms change from a metallic to a semiconducting behavior. However, the metallic behavior is kept when the nanosheets are functionalized with B or Al atoms. Finally, by placing our results within the context of silicon-based systems previous investigations, we could envision potential applications for those nanosheets in van der Waals heterostructures, alkali-metal ion batteries, UV-light devices, and thermoelectric materials.

==> introduction/rascunhos_textos.tex <==



\section{PAPERS}
\subsection{silicene}
(2009) Two- and One-Dimensional Honeycomb Structures of Silicon and Germanium. First-principles calculations of structure optimization, phonon modes, and finite temperature molecular dynamics predict that silicon and germanium can have stable, two-dimensional, low-buckled, honeycomb structures.

(2010) Epitaxial growth of a silicene sheet. The experimental evidence of a silicene sheet (graphenelike structure) epitaxially grown on a close-packed silver surface [Ag(111)]
https://doi.org/10.1063/1.3524215


(2013) Buckled Silicene Formation on Ir(111). This work provides an explanation for the formation of the buckled silicene sheet.
https://pubs.acs.org/doi/pdf/10.1021/nl304347w

(2013) Structural, electronic, and optical properties of hydrogenated few-layer silicene: Size and stacking effects.

https://doi.org/10.1063/1.4820566

(2020) Multilayer silicene: Structure, electronics, and mechanical property

https://doi.org/10.1016/j.commatsci.2019.109354


\subsection{chemical functionalization silicene}

(2013) Adsorption and absorption of boron, nitrogen, aluminum, and phosphorus on silicene: Stability and electronic and phonon properties

https://doi.org/10.1103/PhysRevB.87.085444

(2013) Density Functional Theory Study of the Silicene-like SiX and XSi3 (X = B, C, N, Al, P) Honeycomb Lattices: The Various Buckled Structures and Versatile Electronic Properties.

https://doi.org/10.1021/jp407666m

(2016) Two-dimensional SiS layers with promising electronic and optoelectronic properties: theoretical prediction. 

https://doi.org/10.1021/acs.nanolett.5b04341

(2017) Ab initio prediction and characterization of phosphorene-like SiS and SiSe as anode materials for sodium-ion batteries. 

https://doi.org/10.1016/j.scib.2017.03.026




\subsection{LIB}

(2013) Adsorption and Diffusion of Lithium on Layered Silicon for Li-Ion Storage.

https://doi.org/10.1021/nl400830u

(2017) Silicene: A Promising Anode for Lithium-Ion Batteries. The electrochemical performance of silicene is reviewed in terms of both theoretical predictions and experimental measurements, and finally, its challenges and outlook are considered.

 https://doi.org/10.1002/adma.201606716
 

\textbf{[THES MOST IMPORTANT PAPER] (2018) Few‐Layer Silicene Nanosheets with Superior Lithium‐Storage Properties.} 

 https://doi.org/10.1002/adma.201800838
 
 (2020) Electrochemical Dilatometry of Si-Bearing Electrodes: Dimensional Changes and Experiment Design. For silicon-rich anodes, the electrode dilation can be higher than 300\%, and the expansion profile consists of a combination of slow swelling at low lithiation followed by an accelerated increase at higher lithium contents.
 
 https://iopscience.iop.org/article/10.1149/1945-7111/abd465
 
 (2020) Stable high-capacity and high-rate silicon-based lithium battery anodes upon two-dimensional covalent encapsulation. Markedly distinct from existing techniques of battery fabrication, the involved two-dimensional, covalent binding creates a robust and efficient contact between the silicon and electrically conductive media, enabling stable and fast electron as well as ion transport from and to the silicon. 
 
 https://www.nature.com/articles/s41467-020-17686-4
 
 \subsection{LIB/SIB}
 (2017) Recent advances in inorganic 2D materials and their applications in lithium and sodium batteries.

DOI: 10.1039/C6TA09831B

 (2020) Review on comprehending and enhancing the initial Coulombic efficiency of anode materials in lithium-ion/sodium-ion batteries.
 
 https://doi.org/10.1016/j.nanoen.2020.105143
 
Xenes as an Emerging D Monoelemental Family: 
Fundamental Electrochemistry and Energy Applications.
https://onlinelibrary.wiley.com/doi/epdf/10.1002/adfm.202002885

 \subsection{SIB}
\textbf{(2020) Prospects in anode materials for sodium ion batteries - A review}

https://doi.org/10.1016/j.rser.2019.109549


 
  \subsection{KIB}
 
 (2017) Phosphorus-Based Alloy Materials for Advanced Potassium-Ion Battery Anode
 
 https://doi.org/10.1021/jacs.6b12185
 
 (2017) Potassium‐Ion Battery Anode Materials Operating through the Alloying–Dealloying Reaction Mechanism
 
  https://doi.org/10.1002/adfm.201703857
 
 \textbf{(2020) Advancements and Challenges in Potassium Ion Batteries: A Comprehensive Review.}
  https://doi.org/10.1002/adfm.201909486

\subsection{KIB/SIB}  
Potential of B/Al‐Doped Silicene Electrodes in Na/K‐Ion Batteries

https://doi.org/10.1002/adts.201800017

\textbf{(2020) A Mini-Review: MXene composites for sodium/potassium-ion batteries}

DOI: 10.1039/D0NR04111D

\subsection{LIB/SIB/KIB (AIBS)}
(2019) Recent Research on Strategies to Improve Ion Conduction in Alkali Metal‐Ion Batteries

https://doi.org/10.1002/batt.201800147

(2020) Transition metal dichalcogenides for alkali metal ion batteries: engineering strategies at the atomic level.

DOI: 10.1039/C9EE03549D

(2020) Recent advances and perspectives of 2D silicon: Synthesis and application for energy storage and conversion

https://www.sciencedirect.com/science/article/pii/S2405829720302713

\subsection{Results idea}
(2019) III–VI van der Waals heterostructures for sustainable energy related applications.
DOI: 10.1039/C9NR00421A

(2016) The development of two dimensional group IV chalcogenides, blocks for van der Waals heterostructures
https://doi.org/10.1039/C5NR06871A

Ab initio study of a 2D h-BAs monolayer: a promising anode material for alkali-metal ion batteries.
https://pubs.rsc.org/en/content/articlelanding/2019/cp/c9cp03242h/unauth#!divAbstract

Ab initio prediction of two-dimensional Si3C enabling high specific capacity as an anode material for Li/Na/K-ion batteries
https://pubs.rsc.org/en/content/articlehtml/2020/ta/c9ta11589g

\subsection{Same structure}
Novel Phases of Semi-Conducting Silicon Nitride Bilayer: A First-Principle Study

https://arxiv.org/abs/1707.02819

Structural, electrical, and Rashba properties of monolayer Janus Si2XY (X,Y =P, As, Sb, and Bi)
https://journals.aps.org/prb/abstract/10.1103/PhysRevB.103.165404.

Computational discovery andcharacterization of polymorphic twodimensional IV–V materials

https://aip.scitation.org/doi/pdf/10.1063/1.4967433

High-pressure melt growth and transport properties of SiP, SiAs, GeP, and GeAs 2D layered semiconductors

https://www.sciencedirect.com/science/article/pii/S0022024816300914?via%3Dihub

Structural, vibrational, and electronic properties of single-layer hexagonal crystals
of group IV and V elements.

https://journals.aps.org/prb/pdf/10.1103/PhysRevB.98.045431

Potential SiX (X = N, P, As, Sb, Bi) homo-bilayers for visible-light photocatalyst applications, DOI: 10.1039/D1CY00304F. Artigo com building blocks da \ce{Si2N2} e \ce{Si2P2} que podemos usar nessa parte de sugestão de futuros estudos com nossas estruturas. Tem a energia de formação negativa nesse artigo dessas homo-bilayers, pode ser útil.

==> results/suppinfo/suppinfo.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% The same is true for Supporting Information, which should use the
%% suppinfo environment.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{suppinfo}


\end{suppinfo}
